Understanding density driven errors for reaction barrier heights

Delocalization errors, such as charge-transfer and some self-interaction errors, plague computationally-efficient and otherwise-accurate density functional approximations (DFAs). Evaluating a semi-local DFA non-self-consistently on the Hartree-Fock (HF) density is often recommended as a computationally cheap remedy for delocalization errors. For sophisticated meta-GGAs like SCAN, this approach can achieve remarkable accuracy. When this HF-DFT (or DFA@HF) significantly improves over the DFA, it is often presumed that the HF density is more accurate than the self-consistent DFA density. By applying the metrics of density-corrected density functional theory (DFT), we show that HF-DFT works for barrier heights by making a localizing charge transfer error or density over-correction, thereby producing a somewhat-reliable cancellation of density- and functional-driven errors for the energy. A quantitative analysis of the charge transfer errors in a few transition states confirms this trend. We do not have the exact functional and exact densities that are needed to evaluate the exact density- and functional-driven errors for the large BH76 database of barrier heights. Instead, we have identified and used three non-local proxy functionals (the SCAN 50% global hybrid, the range-separated hybrid LC-$\omega$PBE, and SCAN-FLOSIC) and their self-consistent densities. These functionals yield reasonably accurate self-consistent barrier heights, and their self-consistent total energies are nearly piecewise linear in fractional electron number - two important points of similarity to the exact functional. We argue that density-driven errors of the energy in a self-consistent density functional calculation are second-order in the density error, and that large density-driven errors arise primarily from incorrect electron transfers over length scales larger than the diameter of an atom.

==> tables/LSDA_BH76_DC_DFT.tex <==
\begin{longtable}{ll|rr|rr|rr}
  \caption{
Functional (FE) and density error (DE) metrics for LSDA on the BH76 set.
Each set of two columns uses a different proxy for the exact functional as in Table V of the main text.
Error statistics are reported in the bottom three rows.
The reaction index used by the GMTKN and the symbolic index are given in the first two columns.}
  \label{tab:dc_dft_BH76_LSDA}
\toprule
 &  & \multicolumn{2}{c}{SCAN-FLOSIC} & \multicolumn{2}{c}{\lcwpbe{}} & \multicolumn{2}{c}{SX-0.5} \\ 
Index & Reaction & FE & DE & FE & DE & FE & DE \\ 
  \endfirsthead
\toprule
\toprule
 &  & \multicolumn{2}{c}{SCAN-FLOSIC} & \multicolumn{2}{c}{\lcwpbe{}} & \multicolumn{2}{c}{SX-0.5} \\ 
Index & Reaction & FE & DE & FE & DE & FE & DE \\ 
  \endhead
\toprule
1 & H + N$_2$O $\rightarrow$ N$_2$ + OH & 4.69 & -13.10 & -13.76 & -1.60 & -8.84 & -2.72 \\  
2 & 1 reverse & -46.98 & -19.50 & -42.44 & -3.26 & -50.06 & -5.11 \\  
3 & H + HF $\rightarrow$ HF + H & -22.34 & -8.33 & -21.36 & -0.81 & -18.33 & -1.04 \\  
4 & 3 reverse & -22.34 & -8.33 & -21.36 & -0.81 & -18.33 & -1.04 \\  
5 & H + HCl $\rightarrow$ HCl + H & -11.91 & -3.95 & -14.59 & -1.64 & -8.52 & -2.53 \\  
6 & 5 reverse & -11.91 & -3.95 & -14.59 & -1.64 & -8.52 & -2.53 \\  
7 & CH$_3$F + H $\rightarrow$ CH$_3$ + HF & -16.49 & -8.44 & -17.51 & -1.54 & -14.38 & -2.12 \\  
8 & 7 reverse & -19.26 & -9.06 & -23.40 & -1.90 & -24.38 & -2.97 \\  
9 & F$_2$ + H $\rightarrow$ F + HF & 6.13 & -17.41 & -12.68 & -3.40 & 5.61 & -14.13 \\  
10 & 9 reverse & -17.16 & -18.29 & -29.39 & -3.74 & -29.65 & -15.18 \\  
11 & CH$_3$ + ClF $\rightarrow$ CH$_3$F + Cl & -7.03 & -11.61 & -17.97 & -3.00 & -12.84 & -5.58 \\  
12 & 11 reverse & -10.45 & -12.82 & -22.03 & -8.87 & -19.77 & -11.32 \\  
13 & CH$_3$F + F$^-$ $\rightarrow$ FCH$_3$ + F$^-$ & -10.80 & -2.42 & -10.57 & -1.65 & -9.15 & -2.80 \\  
14 & 13 reverse & -10.80 & -2.42 & -10.57 & -1.65 & -9.15 & -2.80 \\  
15 & CH$_3$F $\hdots$ F$^-$ $\rightarrow$ FCH$_3$ $\hdots$ F$^-$ & -8.09 & -1.67 & -6.80 & -0.77 & -7.24 & -1.79 \\  
16 & 15 reverse & -8.09 & -1.67 & -6.80 & -0.77 & -7.24 & -1.79 \\  
17 & CH$_3$Cl + Cl$^-$ $\rightarrow$ ClCH$_3$ + Cl$^-$ & -7.43 & -1.69 & -12.25 & -2.65 & -7.54 & -2.41 \\  
18 & 17 reverse & -7.43 & -1.69 & -12.25 & -2.65 & -7.54 & -2.41 \\  
19 & CH$_3$Cl $\hdots$ Cl$^-$ $\rightarrow$ ClCH$_3$ $\hdots$ Cl$^-$ & -5.56 & -1.16 & -9.28 & -1.67 & -5.93 & -1.62 \\  
20 & 19 reverse & -5.56 & -1.16 & -9.28 & -1.67 & -5.93 & -1.62 \\  
21 & CH$_3$Cl + F$^-$ $\rightarrow$ CH$_3$F + Cl$^-$ & -4.33 & -2.58 & -10.92 & -2.33 & -5.25 & -2.66 \\  
22 & 21 reverse & -13.17 & -3.40 & -10.70 & -2.25 & -11.28 & -3.46 \\  
23 & F$^-$ $\hdots$ CH$_3$Cl $\rightarrow$ CH$_3$F $\hdots$ Cl$^-$ & -2.38 & -0.77 & -5.70 & -0.69 & -3.09 & -1.02 \\  
24 & 23 reverse & -11.24 & -3.03 & -8.44 & -1.71 & -9.76 & -2.96 \\  
25 & CH$_3$F + OH$^-$ $\rightarrow$ HOCH$_3$ + F$^-$ & -11.10 & -2.37 & -10.33 & -1.62 & -9.39 & -2.59 \\  
26 & 25 reverse & -10.25 & -2.37 & -12.91 & -2.02 & -10.94 & -2.62 \\  
27 & CH$_3$F $\hdots$ OH$^-$ $\rightarrow$ HOCH$_3$ $\hdots$ F$^-$ & -8.71 & -1.86 & -7.07 & -0.98 & -7.67 & -1.84 \\  
28 & 27 reverse & -2.91 & -2.04 & -3.32 & -1.45 & -4.27 & -2.11 \\  
29 & H + N$_2$ $\rightarrow$ HN$_2$ & -6.18 & -6.59 & -12.95 & -1.56 & -6.41 & -3.86 \\  
30 & 29 reverse & -6.54 & -2.88 & -3.09 & -0.62 & -2.87 & -1.45 \\  
31 & H + CO $\rightarrow$ HCO & -4.99 & -1.96 & -8.08 & -1.86 & -4.40 & -2.02 \\  
32 & 31 reverse & -0.32 & -0.71 & 1.57 & -1.30 & 1.87 & -0.74 \\  
33 & H + C$_2$H$_4$ $\rightarrow$ CH$_3$CH$_2$ & -0.54 & -1.89 & -5.23 & -2.20 & 1.78 & -3.64 \\  
34 & 33 reverse & -6.55 & -1.40 & -6.88 & -1.46 & -5.17 & -2.72 \\  
35 & C$_2$H$_4$ + CH$_3$ $\rightarrow$ CH$_3$CH$_2$CH$_2$ & -3.93 & -3.44 & -9.16 & -3.86 & -3.74 & -5.75 \\  
36 & 35 reverse & -1.44 & -1.85 & -3.36 & -2.72 & 1.07 & -4.50 \\  
37 & HCN $\rightarrow$ HNC & -0.77 & -2.06 & -1.91 & -0.17 & -1.01 & -0.71 \\  
38 & 37 reverse & -2.49 & -2.06 & -2.69 & -0.10 & -3.22 & -0.69 \\  
39 & H + HCl $\rightarrow$ H$_2$ + Cl & -5.19 & -1.87 & -7.68 & -1.32 & -2.32 & -2.16 \\  
40 & 39 reverse & -14.95 & -3.61 & -15.81 & -7.01 & -14.19 & -7.39 \\  
41 & OH + H$_2$ $\rightarrow$ H + H$_2$O & -20.52 & -5.58 & -19.75 & -1.76 & -20.20 & -4.01 \\  
42 & 41 reverse & 3.92 & -4.72 & -8.15 & -1.68 & -0.52 & -4.14 \\  
43 & CH$_3$ + H$_2$ $\rightarrow$ CH$_4$ + H & -12.07 & -2.41 & -14.44 & -1.30 & -14.19 & -1.77 \\  
44 & 43 reverse & -5.52 & -1.22 & -8.77 & -1.20 & -4.24 & -1.64 \\  
45 & CH$_4$ + OH $\rightarrow$ CH$_3$ + H$_2$O & -23.18 & -4.86 & -20.89 & -1.59 & -21.69 & -3.79 \\  
46 & 45 reverse & -5.29 & -5.19 & -14.96 & -1.61 & -11.96 & -4.04 \\  
47 & H$_2$ + H $\rightarrow$ H + H$_2$ & -7.99 & -1.51 & -9.96 & -0.78 & -6.48 & -1.09 \\  
48 & 47 reverse & -7.99 & -1.51 & -9.96 & -0.78 & -6.48 & -1.09 \\  
49 & NH$_3$ + OH $\rightarrow$ NH$_2$ + H$_2$O & -26.96 & -6.16 & -25.43 & -1.88 & -26.21 & -4.39 \\  
50 & 49 reverse & -19.22 & -5.84 & -22.32 & -1.81 & -21.13 & -4.31 \\  
51 & CH$_3$ + HCl $\rightarrow$ CH$_4$ + Cl & -11.44 & -1.61 & -13.66 & -1.70 & -12.70 & -2.11 \\  
52 & 51 reverse & -14.65 & -2.16 & -16.13 & -7.29 & -14.62 & -7.21 \\  
53 & C$_2$H$_6$ + OH $\rightarrow$ C$_2$H$_5$ + H$_2$O & -22.91 & -6.11 & -21.45 & -2.29 & -21.85 & -4.74 \\  
54 & 53 reverse & -3.69 & -5.72 & -13.81 & -1.80 & -10.34 & -4.31 \\  
55 & F + H$_2$ $\rightarrow$ H + HF & -17.54 & -9.73 & -18.65 & -2.74 & -18.29 & -7.64 \\  
56 & 55 reverse & 15.43 & -8.31 & -4.09 & -2.66 & 7.69 & -7.59 \\  
57 & O + CH$_4$ $\rightarrow$ OH + CH$_3$ & -22.30 & -3.44 & -19.14 & -1.60 & -21.35 & -3.26 \\  
58 & 57 reverse & -14.61 & -3.28 & -16.30 & -1.42 & -15.47 & -2.65 \\  
59 & H + PH$_3$ $\rightarrow$ H$_2$ + PH$_2$ & -6.36 & -1.70 & -8.63 & -1.68 & -4.85 & -1.58 \\  
60 & 59 reverse & -10.11 & -2.40 & -12.26 & -1.85 & -10.99 & -1.65 \\  
61 & H + OH $\rightarrow$ O + H$_2$ & -10.15 & -2.77 & -11.54 & -0.91 & -6.96 & -2.17 \\  
62 & 61 reverse & -24.39 & -4.13 & -20.04 & -1.19 & -22.79 & -2.91 \\  
63 & H + H$_2$S $\rightarrow$ H$_2$ + HS & -7.03 & -1.35 & -9.19 & -1.41 & -5.28 & -1.48 \\  
64 & 63 reverse & -13.60 & -2.78 & -15.29 & -6.20 & -14.36 & -6.03 \\  
65 & O + HCl $\rightarrow$ OH + Cl & -26.10 & -10.53 & -24.44 & -6.83 & -25.35 & -9.50 \\  
66 & 65 reverse & -21.61 & -10.91 & -24.07 & -12.24 & -21.40 & -13.99 \\  
67 & NH$_2$ + CH$_3$ $\rightarrow$ NH + CH$_4$ & -15.80 & -2.75 & -16.35 & -1.80 & -15.75 & -2.49 \\  
68 & 67 reverse & -16.12 & -2.29 & -16.38 & -1.97 & -16.13 & -2.81 \\  
69 & NH$_2$ + C$_2$H$_5$ $\rightarrow$ NH + C$_2$H$_6$ & -14.42 & -2.27 & -15.70 & -1.44 & -15.06 & -2.03 \\  
70 & 69 reverse & -16.09 & -2.54 & -17.44 & -2.13 & -17.22 & -3.03 \\  
71 & NH$_2$ + C$_2$H$_6$ $\rightarrow$ NH$_3$ + C$_2$H$_5$ & -20.73 & -3.20 & -19.50 & -1.95 & -19.25 & -3.04 \\  
72 & 71 reverse & -9.25 & -3.14 & -14.96 & -1.53 & -12.82 & -2.69 \\  
73 & NH$_2$ + CH$_4$ $\rightarrow$ NH$_3$ + CH$_3$ & -20.14 & -2.54 & -18.69 & -1.61 & -18.59 & -2.58 \\  
74 & 73 reverse & -10.00 & -3.19 & -15.87 & -1.70 & -13.94 & -2.91 \\  
75 & \textit{s-trans cis-}C$_5$H$_8$ $\rightarrow$ \textit{s-trans cis-}C$_5$H$_8$ & -30.48 & -1.37 & -16.87 & 1.30 & -16.73 & 0.84 \\  
76 & 75 reverse & -30.48 & -1.37 & -16.87 & 1.30 & -16.73 & 0.84 \\ \hline 
 & Mean & -11.53 & -4.45 & -13.76 & -2.14 & -11.61 & -3.52 \\ 
 & Mean Abs. & 12.32 & 4.45 & 13.80 & 2.21 & 12.08 & 3.56 \\ 
 & Variance & 221.86 & 36.53 & 239.00 & 8.65 & 213.50 & 21.58 \\ \hline 
\end{longtable}

==> tables/SX-x_nelec_error.tex <==
\begin{ruledtabular}

\begin{table}
    \centering
    \begin{tabular}{rrr}
$x$ & BH Error (kcal/mol) & $\Delta N$ (CH$_3$ side) \\ \hline
0.00 & 12.55 & -0.0702 \\
0.10 & 12.48 & -0.0645 \\
0.25 & 12.09 & -0.0539 \\
0.50 & 10.33 & -0.0302 \\
0.75 & 6.85 & -0.0013 \\
0.85 & 5.03 & 0.0105 \\
1.00 & 1.93 & 0.0270 \\ \hline
@HF & 0.94 & 0.0357 \\
    \end{tabular}
    \caption{Barrier height (BH) errors and charge transfer errors $\Delta N$ for the reaction CH$_3$ + FCl $\rightarrow$ CH$_3$F + Cl. 
    The charge transfer or density errors are evaluated on the CH$_3$ side of the transition state. 
    Self-consistent densities are taken from SX-$x$, eq \ref{eq:SX-x}, and BH errors are SCAN@SX-$x$.}
    \label{tab:SCAN_at_SX_DE}
\end{table}

\end{ruledtabular}

==> tables/bh24_w_sic.tex <==
\begin{ruledtabular}
    \begin{table}[ht]
        \centering
        \begin{tabular}{l|rrrr}
 & \multicolumn{4}{c}{Hydrogen transfer (HTBH6)} \\
DFA & @DFA & -FLOSIC & @FLOSIC & @HF \\ \hline
LSDA & (-)18.10 & (-5.00)5.04 & (-)14.90 & (-)9.96 \\
PBE & (-9.60)9.61 & (0.38)4.21 & (-6.30)6.34 & (-)3.27 \\
SCAN & (-)7.90 & (-0.58)2.80 & (-6.60)6.57 & (-)3.25 \\ \hline
& \multicolumn{4}{c}{Heavy atom transfer (HABH6)} \\
LSDA & (-)23.02 & (-0.62)4.46 & (-)12.05 & (-6.18)8.09 \\
PBE & (-)14.38 & (2.16)7.36 & (-)5.67 & (-0.78)4.90 \\
SCAN & (-)11.52 & (2.33)5.00 & (-)5.40 & (-2.33)2.96 \\ \hline
 & \multicolumn{4}{c}{Unimolecular and association (UABH6)} \\
LSDA & (-)5.60 & (3.94)6.28 & (-2.64)3.32 & (0.58)1.98 \\
PBE & (-)3.31 & (3.44)3.95 & (-0.29)0.98 & (10.9)1.83 \\
SCAN & (-3.07)3.64 & (0.88)3.59 & (-1.80)2.80 & (-0.80)2.44 \\ \hline
 & \multicolumn{4}{c}{Nucleophilic substitution (NSBH6)} \\
LSDA & (-)8.84 & 7.65 & (-)5.00 & 0.79 \\
PBE & (-)7.45 & 7.54 & (-)3.73 & (-2.53)3.85 \\
SCAN & (-)6.79 & (3.23)3.84 & (-)4.54 & (0.76)0.99 \\ \hline
 & \multicolumn{4}{c}{BH24} \\
LSDA & (-)13.89 & (1.74)5.86 & (-8.70)8.82 & (-3.70)5.22 \\
PBE & (-8.70)8.69 & (3.38)5.76 & (-4.00)4.18 & (-1.37)3.46 \\
SCAN & (-7.30)7.46 & (1.48)3.80 & (-4.60)4.83 & (-1.38)2.41 \\
       \end{tabular}
    \caption{ Mean (ME) and mean absolute errors (MAE) in the BH24 set \cite{zheng2007} set of reaction BHs, with its subsets.
    If the ME is the negative of the MAE (to stated precision), then only the negative sign is given in parenthesis.
    If the ME and MAE are equal (to stated precision), no parenthetical value is given.
    The first column, ``@DFA'', gives self-consistent values; the second column, ``-FLOSIC'', gives self-consistent DFA-FLOSIC values.
    The ``@FLOSIC'' column indicates a DFA was evaluated non-self-consistently on its (self-consistent) DFA-FLOSIC density.
    The ``@HF'' column indicates that a DFA was evaluated non-self-consistently on the HF density.
    \label{tab:bh24}}
    \end{table}
\end{ruledtabular}

==> tables/bh76_sic.tex <==
\begin{ruledtabular}
\begin{table*}
  \centering
  \caption{BH76 error statistics (in kcal/mol) using the FLOSIC code and its default NRLMOL basis set \cite{porezag1999}. 
  The first four columns (after the ME/MAE column) present self-consistent DFA results.
  The second set of four columns present self-consistent DFA-FLOSIC calculations.
  The last set of four columns presents the DFA evaluated non-selfconsistently on its self-consistent DFA-FLOSIC density.}
    \begin{tabular}{lrrrr|rrrr|rrrr}
          & \multicolumn{4}{c|}{DFA} & \multicolumn{4}{c|}{-PZSIC} & \multicolumn{4}{c}{ DFA@PZSIC} \\
          & LSDA & PBE & SCAN  & r$^2$SCAN & LSDA  & PBE & SCAN & r$^2$SCAN & LSDA & PBE & SCAN  & r$^2$SCAN \\
          \hline
    ME & -15.36 & -9.88 & -7.74 & -7.24 & 0.26  & 3.04  & 0.61  & 1.34  & -10.93 & -5.02 & -5.76 & -5.23 \\
    MAE & 15.46 & 10.49 & 7.81  & 7.30 & 5.70 & 5.26  & 3.79  & 3.54 & 11.17 & 5.34  & 5.85  & 5.31 \\
    \end{tabular}
  \label{tab:bh76_sic}
\end{table*}
\end{ruledtabular}
